SoK: Reducing the Vulnerability of Fine-tuned Language Models to Membership Inference Attacks

Natural language processing models have experienced a significant upsurge in recent years, with numerous applications being built upon them. Many of these applications require fine-tuning generic base models on customized, proprietary datasets. This fine-tuning data is especially likely to contain personal or sensitive information about individuals, resulting in increased privacy risk. Membership inference attacks are the most commonly employed attack to assess the privacy leakage of a machine learning model. However, limited research is available on the factors that affect the vulnerability of language models to this kind of attack, or on the applicability of different defense strategies in the language domain. We provide the first systematic review of the vulnerability of fine-tuned large language models to membership inference attacks, the various factors that come into play, and the effectiveness of different defense strategies. We find that some training methods provide significantly reduced privacy risk, with the combination of differential privacy and low-rank adaptors achieving the best privacy protection against these attacks.

==> tables/dp_ablation.tex <==
\begin{table*}[h]
\centering
\caption{Ablation Study for DP-SGD. \\The number in parentheses represents the standard deviation across 20 experiments.}
\label{tab:dp_ablation}
\begin{tabular}{l|ccccccccc}
\hline\hline
                     & \multicolumn{3}{c}{CoLA}                                                                                                                                            & \multicolumn{3}{c}{Rotten Tomatoes}                                                                                                                                 & \multicolumn{3}{c}{Yahoo Answers}                                                                                                                                   \\ \hline
                     & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} \\ \hline
Base Model           & 57.44(1.07)                                        & 8.48(1.77)                                              & 83.50                                                & 58.65(1.58)                                        & 5.32(1.40)                                              & 90.15                                                & 53.57(1.68)                                        & 0.31(0.31)                                              & 72.77                                                \\
Gradient Noise       & 57.75(1.68)                                        & 7.96(1.68)                                              & 85.04                                                & 56.81(1.63)                                        & 5.26(0.85)                                              & 88.06                                                & 51.53(0.97)                                        & 0.31(0.21)                                              & 72.37                                                \\
Gradient Clipping    & 51.26(0.88)                                        & 3.37(0.77)                                              & 73.63                                                & 52.41(1.73)                                        & 1.81(1.00)                                              & 84.89                                                & 52.04(1.14)                                        & 0.31(0.23)                                              & 71.74                                                \\
DP-SGD($\epsilon$=2) & 51.36(0.97)                                        & 2.60(1.10)                                              & 76.41                                                & 50.71(0.87)                                        & 1.52(0.53)                                              & 85.33                                                & 50.02(0.85)                                        & 0.31(0.21)                                              & 66.55                                                \\ \hline\hline
\end{tabular}
\end{table*}

==> tables/dp_mia_acc.tex <==
\begin{tabular}{cccccccccc}
\hline\hline
                  & \multicolumn{9}{c}{MIA Acc}                                                                                                                                                                                                           \\ \hline
                  & \multicolumn{3}{c}{CoLA}                                                & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Rotten \\ Tomatoes\end{tabular}} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Yahoo \\ Answers\end{tabular}} \\
                  & \begin{tabular}[c]{@{}c@{}}W.o.\\  Privacy\end{tabular} & $\epsilon$=2 & $\epsilon$=3 & \begin{tabular}[c]{@{}c@{}}W.o. \\ Privacy\end{tabular}    & $\epsilon$=2   & $\epsilon$=3   & \begin{tabular}[c]{@{}c@{}}W.o.\\  Privacy\end{tabular}   & $\epsilon$=2   & $\epsilon$=3  \\ \hline
Base Model        &        63.3                                                 & -     & -     &                                                     64.6       & -       & -       &                                     54.6  & -       & -      \\
Gradient noise    &    62.4    & -     & -     &                                                   61.8         & -       & -       &                                                           & -       & -      \\
Gradient Clipping &        54.0       & -     & -     &                                                    55.8        &   -      &     -    &                                                           &     -    &    -    \\
DP-SGD   & -                                                       &       &       & -                                                          &    52.0     &    51.6     & -                                                         &         &        \\
LoRA+DP-SGD       & -                                                       &   51.6    &  52.4    & -                                                          &     52.8     &    53.0     & -                                                         &    52.6     &   52.6     \\ \hline\hline
\end{tabular}



==> tables/dp_model_acc.tex <==
\begin{tabular}{cccccccccc}
\hline\hline
                  & \multicolumn{9}{c}{Model Acc}                                                                                                                                                                                                           \\ \hline
                  & \multicolumn{3}{c}{CoLA}                                                & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Rotten \\ Tomatoes\end{tabular}} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Yahoo \\ Answers\end{tabular}} \\
                  & \begin{tabular}[c]{@{}c@{}}W.o.\\  Privacy\end{tabular} & $\epsilon$=2 & $\epsilon$=3 & \begin{tabular}[c]{@{}c@{}}W.o. \\ Privacy\end{tabular}    & $\epsilon$=2   & $\epsilon$=3   & \begin{tabular}[c]{@{}c@{}}W.o.\\  Privacy\end{tabular}   & $\epsilon$=2   & $\epsilon$=3  \\ \hline
Base Model        &      83.5                                                   & -     & -     &                                                      90.15      & -       & -       &                                          72.77                 & -       & -      \\
Gradient noise    &        85.04                                                 & -     & -     &                                                    88.06        & -       & -       &                                                           & -       & -      \\
Gradient Clipping &        73.63           & -     & -     &                                                    84.89       &      -   &     -    &                                                           &     -    &    -    \\
DP-SGD            & -                                                       &       &       & -                                                          &   85.33      &    84.80      & -                                                         &         &        \\
LoRA+DP-SGD       & -                                                       &   77.85    &   79.76    & -                                                          &    88.55     &   86.49      & -                                                         &    70.39     &     70.33   \\ \hline\hline
\end{tabular}



==> tables/mitagation_categories.tex <==
\begin{table}[h]
\begin{tabular}{cccc}
\hline\hline
                    & \begin{tabular}[c]{@{}c@{}}Reduced Model\\ Performance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Increased \\ Run-Time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Different\\ Hyper-Parameters\end{tabular} \\ \hline
MI-Pruning          &                                                                     &                                                               &                                                                      \\
Mem-Guard           &                                                                     &                                                               &                                                                      \\
DP-SGD              &                                                                     &                                                               &                                                                      \\
FP-DP               &                                                                     &                                                               &                                                                      \\
DP-SGD + LoRA      &                                                                     &                                                               &                                                                      \\
\hline\hline
\end{tabular}
\end{table}

==> tables/old/best_method_tables.tex <==
\begin{table*}[!h]
\centering
\caption{A summery of the leading methods for preventing MIA attacks on LLMs and their combinations. \\The number in parentheses represents the standard deviation across 20 experiments.}
\label{tab:sum}
\begin{tabular}{l|ccccccccc}
\hline\hline
                               & \multicolumn{3}{c}{CoLA}                                                                                                                                            & \multicolumn{3}{c}{Rotten Tomatoes}                                                                                                                                 & \multicolumn{3}{c}{Yahoo Answers}                                                                                                                                   \\ \hline
Method                         & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} \\ \hline
Roberta Base                   & 57.44(1.07)                                        & 8.48(1.77)                                              & 83.5                                                 & 58.65(1.58)                                        & 5.32(1.40)                                              & 90.15                                                & 53.57(1.68)                                        & 0.31(0.31)                                              & 72.77                                                \\
Roberta Base + Large Batch     & 55.60(1.59)                                        & 6.75(1.43)                                              & 81.97                                                & 53.62(1.84)                                        & 3.93(1.34)                                              & 89.0                                                 & 52.29(1.30)                                        & 0.36(0.22)                                              & 73.33                                                \\
LoRA                           & 50.97(1.00)                                        & 3.19(1.110)                                             & 81.39                                                & 50.09(1.26)                                        & 3.03(1.15)                                              & 87.80                                                & 50.36(1.09)                                        & 0.31(0.24)                                              & 72.52                                                \\
Distilled + LoRA               & 50.25(1.24)                                        & 2.87(0.97)                                              & 80.72                                                & 50.51(1.02)                                        & 2.18(0.76)                                              & 86.77                                                & 50.36(1.09)                                        & 0.21(0.13)                                              & 71.76                                                \\
Distilled + LoRA + Large Batch & 51.51(1.17)                                        & 2.87(0.97)                                              & 79.19                                                & 50.66(0.78)                                        & 2.18(0.76)                                              & 86.30                                                & 51.08(0.71)                                        & 0.36(0.17)                                              & 71.41                                                \\
DP-LoRA($\epsilon$=2)          & 51.42(0.92)                                        & 1.64(0.52)                                              & 77.85                                                & 50.96(1.02)                                        & 1.22(0.68)                                              & 88.55                                                & 50.44(0.75)                                        & 0.25(0.16)                                              & 70.39                                                \\ \hline\hline
\end{tabular}
\end{table*}

==> tables/old/dp_vs_dp_lora_table.tex <==
\begin{table*}[h]
\centering
\caption{Comparison between DP-SGD (full fine-tuning) and DP-LoRA. \\The number in parentheses represents the standard deviation across 20 experiments.}
\label{tab:dp_vs_dp_lora}
\begin{tabular}{l|ccccccccc}
\hline\hline
                      & \multicolumn{3}{c}{CoLA}                                                                                                                                            & \multicolumn{3}{c}{Rotten Tomatoes}                                                                                                                                 & \multicolumn{3}{c}{Yahoo Answers}                                                                                                                                   \\ \hline
                      & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  ACC\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  ACC\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} \\ \hline
% DP-SGD($\epsilon$=5)  & 51.74(1.18)                                        & 1.63(0.82)                                              & 77.37                                                & 50.85(0.65)                                        & 1.22(0.69)                                              & 85.36                                                & 50.82(0.50)                                        & 0.26(0.17)                                              & 65.25                                                \\
DP-SGD($\epsilon$=2)  & 51.36(0.97)                                        & 2.60(1.10)                                              & 76.41                                                & 50.71(0.87)                                        & 1.52(0.53)                                              & 85.33                                                & 50.02(0.85)                                        & 0.31(0.21)                                              & 66.55                                                \\
% DP-LoRA($\epsilon$=5) & 51.10(1.03)                                        & 2.43(0.94)                                              & 79.00                                                & 50.71(0.90)                                        & 1.80(0.96)                                              & 87.42                                                & 50.91(0.82)                                        & 0.20(0.22)                                              & 69.59                                                \\
DP-LoRA($\epsilon$=2) & 51.42(0.92)                                        & 1.64(0.52)                                              & 77.85                                                & 50.96(1.02)                                        & 1.22(0.68)                                              & 88.55                                                & 50.44(0.75)                                        & 0.25(0.16)                                              & 70.39                                                \\ \hline\hline
\end{tabular}
\end{table*}

==> tables/old/model_size_table.tex <==
\begin{table*}[ht]
\centering
\caption{The effect of reducing the model size on MI attacks success rate. \\The number in parentheses represents the standard deviation across 20 experiments.}
\label{tab:size}
\begin{tabular}{lc|ccccccccc}
\hline\hline
\multicolumn{2}{c|}{}                                                                  & \multicolumn{3}{c}{CoLA}                                                                                                                                            & \multicolumn{3}{c}{Rotten Tomatoes}                                                                                                                                 & \multicolumn{3}{c}{Yahoo Answers}                                                                                                                                   \\ \hline
Method               & \begin{tabular}[c]{@{}c@{}}Trainable\\  Parameters\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}MIA\\  Acc\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR@\\ FPR0.1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model\\  Acc\end{tabular} \\ \hline
Roberta-Base         & 125M                                                            & 57.44(1.07)                                        & 8.48(1.77)                                              & 83.5                                                 & 58.65(1.58)                                        & 5.32(1.40)                                              & 90.15                                                & 53.57(1.68)                                        & 0.31(0.31)                                              & 72.77                                                \\
Unstructured pruning & 100M                                                            & 57.06(1.14)                                        & 7.50(1.35)                                              & 83.79                                                & 56.69(1.02)                                        & 4.89(1.02)                                              & 90.15                                                & 51.36(1.53)                                        & 0.31(0.18)                                              & 72.14                                                \\
GAP Prune            & 87.8M                                                           & 54.06(0.93)                                        & 6.06(0.96)                                              & 81.88                                                & 52.69(1.51)                                        & 3.98(1.75)                                              & 84.4                                                 & 53.02(1.13)                                        & 0.25(0.16)                                              & 72.50                                                \\
Distilled Model      & 82.8M                                                           & 58.08(1.18)                                        & 9.57(2.53)                                              & 81.87                                                & 59.44(1.59)                                        & 4.93(0.84)                                              & 86.49                                                & 53.41(1.76)                                        & 0.20(0.16)                                              & 71.48                                                \\
LoRA                 & 1.5M                                                            & 50.97(1.00)                                        & 3.19(1.11)                                             & 81.39                                                & 50.09(1.26)                                        & 3.03(1.15)                                              & 87.80                                                & 50.36(1.09)                                        & 0.31(0.24)                                              & 72.52                                                \\
Distilled Model+LoRA & 1.3M                                                            & 50.25(1.24)                                        & 2.87(0.97)                                              & 80.72                                                & 50.51(1.02)                                        & 2.18(0.76)                                              & 86.77                                                & 50.36(1.09)                                        & 0.21(0.13)                                              & 71.76                                                \\ \hline\hline
\end{tabular}
\end{table*}
